D3: A Massive Dataset of Scholarly Metadata for Analyzing the State of Computer Science Research

DBLP is the largest open-access repository of scientific articles on computer science and provides metadata associated with publications, authors, and venues. We retrieved more than 6 million publications from DBLP and extracted pertinent metadata (e.g., abstracts, author affiliations, citations) from the publication texts to create the DBLP Discovery Dataset (D3). D3 can be used to identify trends in research activity, productivity, focus, bias, accessibility, and impact of computer science research. We present an initial analysis focused on the volume of computer science research (e.g., number of papers, authors, research activity), trends in topics of interest, and citation patterns. Our findings show that computer science is a growing research field (approx. 15% annually), with an active and collaborative researcher community. While papers in recent years present more bibliographical entries in comparison to previous decades, the average number of citations has been declining. Investigating papers' abstracts reveals that recent topic trends are clearly reflected in D3. Finally, we list further applications of D3 and pose supplemental research questions. The D3 dataset, our findings, and source code are publicly available for research purposes.

==> _take_out.tex <==

\subsection{Publishers and Accessibility}
\textit{Q5. What are the most prominent publishers?}\\
% How are publications distributed by publishers?
\Cref{fig:analysis-publications-by-publishers} shows the share of publishers in \projectName until December 2021.
Springer is the by far the largest publisher of academic literature on computer science with $53.13\%$ of papers being published.
With less than half of Springer's values, IEEE (including IEEE Computer Society), and ACM contain $15.54\%$ and $2.57\%$ of published papers respectively.
The difference between Springer and other publishers show an certain bias in \projectName.
However, considering Springer was founded in 1842 and it is still an active publisher, its prominent representation is expected. 
Other popular names, such as O'Reilly contain as much as $2.05\%$ of computer science papers.
The NLP-focused publisher ACL, only contains $0.58\%$ of the computer science literature, placing itself on the 16\textsuperscript{th} position among the largest publishers.
The remaining publishers not in \Cref{fig:analysis-publications-by-publishers} are similarly equally distributed.
\\\newline
\textit{Q6. How many publications are open access?}\\
% How many publications are accessible to the public?
From the 6 million papers in DBLP, only 1.03 million ($11.77\%$) are marked as open access.
From the open access papers, $37.61\%$ come from arXiv, while Springer, IEEE, and ACM combined sum to less then $1\%$ of papers without a paywall.
The amount of papers under paid modalities (e.g., individual purchase, subscription) shows how much of the science production lays out of reach from society.
It is beyond the scope of this paper to discuss the political and economic implications of a such restrictive attitude.
In addition, we leave to future work the investigation of how many papers are only published in arXiv and the overlap between arXiv and another publishers.
Even though ACL is ranked 16\textsuperscript{th} among the publishers ($x\%$), it contributes with $3.02\%$ of the open access papers.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/num_publications_by_publisher.pdf}
    \caption{The 20 largest publishers and their share (\%) of publications until December 2021.}
    \label{fig:analysis-publications-by-publishers}
\end{figure}



% \textit{Q7. How many citations come from non computer science publications?}\\
% 21 of citations coming from other papers than the dblp
% our dataser consists only in dataset cpomputer to computer.

% Approximately $21\%$ of citations come from papers outside \projectName.
% To compute the percentage of citations coming from computer science publications, we used \semanticScholar and retrieved all citations for papers in DBLP venues.
% As \semanticScholar contains citations coming from papers in different fields, we computed the difference to citations in our citation graph.
% This result shows that computer science is a strongly connected field but also influences other not directly related fields
% \\

% \subsection{Affiliations and Geolocations}
% \textit{Q3. How many institutions/companies publish in DBLP venues?}\\
% \textit{Q4. How is the distribution of countries and cities of authors in DBLP? Which languages are represented in DBLP?}\\
% \textit{Q5. How much collaboration can we observe with authors from other instituations/companies?}\\

% \input{tables/dataset_comparison}


==> tables/dataset_comparison.tex <==
\begin{table*}[htb]
\small
\centering
\begin{tabular}{l c r r r r r} 
\toprule
\textbf{Features} &{} & \textbf{\nlpScholar} & \textbf{NLP4NLP} & \textbf{\nlpExplorer} & \textbf{\projectName} \\

\toprule
Period          & {} & 1965 - 2019 & 1965 - 2015 & 1965 - 2019 & \textbf{1936 - 2021}\\
\#Papers        & {} & 44,896       & 65,000 & 55,565 & \textbf{5,903,710} \\
\#Citations     & {} & 1,210,058    & 325,000 & 723,976 & \textbf{97,831,106} \\
\#Authors       & {} & 18,862       & 50,000 & 39,555 & \textbf{2,889,048} \\
\#Attributes    & {} & 18           & 20 & 29 & \textbf{31}\\
\#Venues        & {} & 20           & 34 & 78 & \textbf{1,921} \\


\bottomrule
\end{tabular}
\caption{Feature comparison between \nlpScholar, \nlpExplorer, \nlpfournlp and \projectName.} \label{tab:dataset_overview_and_comparison}
\end{table*}
